Time-Constrained Model Predictive Control for Autonomous Satellite Rendezvous, Proximity Operations, and Docking

This paper presents a time-constrained model predictive control strategy for the six degree-of-freedom autonomous rendezvous, proximity, operations and docking problem between a controllable "deputy" satellite and an uncontrolled "chief" satellite. The objective is to achieve a docking configuration defined by both the translational and attitudinal states of the deputy relative to the chief, whose dynamics are respectively governed by both the Clohessy-Wiltshire equations and Euler's second law of motion. The proposed control strategy explicitly addresses computational time constraints that are common to state-of-the-art space vehicles. Thus, a time-constrained model predictive control strategy is implemented on a space-grade processor. Although suboptimal with regards to energy consumption when compared to conventional optimal RPO trajectories, it is empirically demonstrated via numerical simulations that the deputy spacecraft still achieves a successful docking configuration while subject to computational time constraints.

==> 4-Problem.tex <==
\section{Problem Statement} \label{sec:problem}

\subsection{Conventional Model Predictive Control} \label{sec:MPC}
In this section, we introduce conventional MPC, then explain how time-constrained MPC differs from it. 
Consider the discrete-time dynamics
%\begin{equation} \label{eq:discreteDyn}
    $x(k+1) = f_d(x(k),u(k))$,
%\end{equation}
where~$x(k) \in \chi \subset \reals^{n}$,~$u(k) \in \U \subset \R^m$, and~$f_d: \chi \times \U \rightarrow \chi$.
The goal of conventional MPC is to solve an optimal control problem at each timestep~$k$ over a finite prediction horizon of length~$N\in\mathbb{N}$, using the current state as the initial state. This process generates
the control sequence~$\textbf{u}^*(k) = \{u^*(k),u^*(k+1),\dots,u^*(N-1)\}$
and the state 
sequence~$\textbf{x}^*(k) = \{x^*(k),x^*(k+1),\dots,x^*(N)\}$. 
Then, the first input in this sequence,~$u^*(k)$, is applied to the system and this process is repeated until the end of the time horizon is reached. 
Formally, the conventional MPC problem that is solved at each time~$k$ is given
next. 
\begin{equation} \label{prob:MPC}
    \begin{split}
        \underset{\textbf{u}(k) \in \U}{\textnormal{minimize}} & \ J( x(k),\textbf{u}(k)) = \sum^{N-1}_{i=k} \ell (x(i),u(i)) \\
        \textnormal{subject to} &\ x(k) = x(0), \\
                                &\  x(i+1) = f_d(x(i),u(i)), \\
                                &\ u_{\min} \leq u(i) \leq u_{\max}, \\
    \end{split}
\end{equation}
where~$\ell : \chi \times \U \rightarrow \reals$
is the cost functional,~$u_{\min}$, $u_{\max} \in \U$ are input limits, and~$\textbf{u}(k)=\{u(k),\dots,u(N-1) \}$.
% The process of solving Problem~\ref{prob:MPC} is shown in Figure~\ref{fig:Loop}.

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.4\textwidth]{Figures/MPCloop.png}
% \caption{A conventional MPC loop. The continuous-time dynamics~$\dot{x}$ determine the initial state~$x(0)$ that is fed into the Receding-Horizon Controller. 
% The resulting
% optimization problem is solved, giving~$\textbf{u}^*(k)$, the first element of which,~$u^*(k)$, is applied to the system. This process repeats until a termination condition is met.} 
% \label{fig:Loop}
% \end{figure}

\subsection{Time-Constrained MPC} \label{sec:tcMPC}
In conventional MPC, Problem~\ref{prob:MPC} is iteratively solved to completion at each time~$k$ by reaching a stopping condition based on the optimality of the solution.
We use~$j_k \in $ to denote the number
of iterations that an optimization algorithm must complete to reach
a stopping condition in the computation of~$\textbf{u}(k)$.
In computationally constrained settings, it cannot be guaranteed that there
is time to execute all~$j_k$ desired iterations because a system input
may be needed before those computations are completed. 
%Moreover, onboard hardware must compute~$j_k$ iterates before reaching completion that can be different for each~$k$, e.g., a gradient descent algorithm must compute~$j_k$ gradient iterates before reaching the stopping condition. However, provided limited onboard computational speed we cannot guarantee that there is sufficient time to solve this problem to completion. 
Therefore, we employ the following time-constrained MPC problem 
%in which we solve the following problem
that has an explicit constraint on~$j_k$. 
\begin{problem}[Time-Constrained MPC] \label{prob:tcMPC}
\begin{small}
\begin{equation} 
    \begin{split}
        \underset{\textbf{u}(k)}{\textnormal{minimize}} & \ J(x(k),\textbf{u}(k)) = \sum^{N-1}_{i=k} \ell (x(i),u(i)) \\
        \textnormal{subject to} &\ x(k) = x(0) \\
                                &\  x(i+1) = f_d(x(i),u(i)), \\
                                &\ u_\min \leq u(i) \leq u_\max, \\
                                & \ j_k \leq j_\max,
    \end{split}
\end{equation}
\end{small}
where~$j_k$ is the number of iterations computed at time~$k$ and~$j_\max$ is the maximum allowable iterations for all~$k$. 
%\mh{Same as above: Make sure every symbol is defined. Should the equation
%with~$x(i+1) = \cdots$ end with~$N-1$ instead of~$N$?}
%\gb{Can I use the same symbols I defined after Problem 1 without redefining them?}
\end{problem}

The constraint~$j_k \leq j_{max}$ models scenarios with limited onboard computational speed in which there is only enough time to complete at most~$j_\max$ iterations. 
A solution to Problem~\ref{prob:tcMPC} at time~$k$ will typically
result in a sub-optimal input and state sequences, i.e.,
%which we denote by~$\tilde{x}$ and~$\tilde{u}$, i.e., 
\begin{equation}
    \begin{split}
        \tilde{\textbf{u}}(k) &= \{\tilde{u}(k),\tilde{u}(k+1),\dots,\tilde{u}(N-1)\} \\
        \tilde{\textbf{x}}(k) &= \{\tilde{x}(k),\tilde{x}(k+1),\dots,\tilde{x}(N)\}, \\
    \end{split}
\end{equation}
respectively. Then, we apply the first input of the resulting input 
sequence, namely~$\tilde{u}(k)$, and repeat this process until the 
end of the time horizon is reached. 
This setup is different from conventional MPC in that we apply a potentially sub-optimal input due to the iteration constraint~$j_k \leq j_{max}$ in Problem~\ref{prob:tcMPC}.
Figure~\ref{fig:mpc} shows the block diagram for our proposed time-constrained MPC strategy.
\begin{figure}[H]
\centering
\includegraphics[width=0.6\textwidth]{Figures/mpcFig.pdf}
\caption{At each time step~$k$ the state~$x_0$ of the ``Dynamic System'' is provided to the ``MPC Controller''. Then, the MPC controller computes a number of algorithmic iterations~$j_k$ to compute the possibly sub-optimal control sequence~\boldmath$\tilde{u}_k$. Then, the first element of the sequence~$\tilde{u}_k$ is applied to the ``Dynamic System''. This process is repeated until a stopping condition is met.
}
\label{fig:mpc}
\end{figure}


Next, we derive the dynamics for the 6DOF ARPOD problem that will be used in our setup and solution to Problem~\ref{prob:tcMPC}. 

\subsection{Dynamics Overview} \label{sec:dynamics}
\begin{figure}[ht]
\centering
\includegraphics[width=0.35\textwidth]{Figures/ARPOD_allframes.pdf}
\caption{The chief (with rotating orbit-fixed frame $\coordframe{O}$) and a deputy (with body-fixed frame $\coordframe{D}$) are orbiting about the Earth with inertial frame $\coordframe{E}$. The dashed lines are the closed orbital trajectories of both spacecraft. The red solid line depicts the rendezvous trajectory from the deputy to the chief as seen in the inertial frame.}
\label{fig:ExclusionZones}
\end{figure}

The objective of this work is to design an autonomous controller such that a deputy spacecraft's translational and attitudinal states converge to a successful docking configuration with the chief, as shown in Figure~\ref{fig:ExclusionZones}. 
Three frames of reference are used: 
\begin{enumerate}
\item {The Earth-Centered Inertial (ECI) frame originating from the Earth's center is denoted $\coordframe{E} := \{\mathbf{\hat{x}_e}, \mathbf{\hat{y}_e}, \mathbf{\hat{z}_e}\}$.}
\item {The Clohessy-Wiltshire (CW) frame is a non-inertial frame attached to the chief satellite, denoted $\mathcal{O} := \{\mathbf{\hat{x}_o}, \mathbf{\hat{y}_o}, \mathbf{\hat{z}_o}\}$. The origin lies at the center of mass of the chief, unless otherwise specified. The $\mathbf{\hat{x}_o}$-axis aligns with the vector pointing from the center of the Earth towards the center of mass of the chief satellite. The $\mathbf{\hat{z}_o}$-axis is in the direction of the orbital angular momentum vector of the chief spacecraft. The $\mathbf{\hat{y}_o}$-axis completes the right-handed orthogonal frame.}
\item{The deputy-fixed frame is a non-inertial body-fixed frame attached to the deputy satellite and denoted $\mathcal{D} := \{\mathbf{\hat{x}_d}, \mathbf{\hat{y}_d}, \mathbf{\hat{z}_d}\}$. The origin is assumed to lie at the center of mass of the deputy, unless otherwise specified. We use the convention that the $\mathbf{\hat{x}_d}$-axis is along the starboard direction, $\mathbf{\hat{y}_d}$ is in the fore direction, and $\mathbf{\hat{z}_d}$ completes the right-handed frame in the topside direction.}
\end{enumerate}
Let $(m_c, \inertia{C})$ and $(m_d, \inertia{D})$ be the mass-inertia pairs of the chief and deputy respectively. We make the following assumptions regarding their relative motion dynamics:

\begin{assumption} \label{as:A1}
    Both the chief and the deputy spacecraft are assumed to be rigid bodies of constant mass
\end{assumption}
\begin{assumption} \label{as:A2}
    The chief-fixed frame is assumed to always align with the orbit-fixed frame $\coordframe{O}$.
\end{assumption}
\begin{assumption} \label{as:A3}
    The chief spacecraft is in an uncontrolled, circular orbit.
\end{assumption}
\begin{assumption} \label{as:A4}
    The distance between the chief and the deputy is much less than the distance between the Earth and the chief.
\end{assumption}
\begin{assumption} \label{as:A5}
    The deputy spacecraft has bi-directional thrusters and external torque-generators installed along the axes aligning with its body-fixed frame.
\end{assumption}
\begin{assumption} \label{as:A6}
    The axes of the deputy-fixed frame are aligned with the principal axes of the deputy body.
\end{assumption}

\begin{comment}
    \begin{description}
\item[A1]{Both the chief and the deputy spacecraft are assumed to be rigid bodies of constant mass.}
\item[A2]{The chief-fixed frame is assumed to always align with the orbit-fixed frame $\coordframe{O}$.}
\item[A3]{The chief spacecraft is in an uncontrolled, circular orbit.}
\item[A4]{The distance between the chief and the deputy is much less than the distance between the Earth and the chief.}
\item[A5]{The deputy spacecraft has bi-directional thrusters and torque-generators installed along the axes aligning with its body-fixed frame.}
\item[A6]{The axes of the deputy-fixed frame are aligned with the principal axes of the deputy body.}
\end{description}
\end{comment}

 The position and velocity of the deputy relative to the chief with respect to the CW frame $\coordframe{O}$ are
\begin{equation}
\delta r^{\coordframe{O}} := (\delta x \ \delta y \ \delta z)^{\top} 
\textnormal{ and }
\delta \dot{r}^{\coordframe{O}} := (\delta \dot{x} \ \delta \dot{y} \ \delta \dot{z})^{\top}.
\end{equation}
Assumptions A3-A5 allow the use of the Clohessy-Wiltshire translational dynamics (see \citep{curtis2013orbital}) with deputy controls, expressed as
\begin{equation}
\label{eq:CWdynamics_translational}
\begin{pmatrix}
\delta \dot{x} \\ \delta \dot{y} \\ \delta \dot{z} \\ \delta \ddot{x} \\ \delta \ddot{y} \\ \delta \ddot{z}
\end{pmatrix}
= \begin{pmatrix}
0 & 0 & 0 & 1 & 0 & 0 \\
0 & 0 & 0 & 0 & 1 & 0 \\
0 & 0 & 0 & 0 & 0 & 1 \\
3n^2& 0 & 0 & 0 & 2n & 0 \\
 0 & 0 & 0 & -2n & 0 & 0 \\
 0 & 0 & -n^2 & 0 & 0 & 0 
\end{pmatrix}
\begin{pmatrix}
\delta x \\ \delta y \\ \delta z \\ \delta \dot{x} \\ \delta \dot{y} \\ \delta \dot{z}
\end{pmatrix} + 
\begin{pmatrix}
\mathbf{0}_{3 \times 3}\\
\frac{1}{m_d}\rotmat{D}{O}
\end{pmatrix}
F^{\coordframe{D}}_d,
\end{equation}
 where the ``mean motion" constant is $n = \sqrt{\frac{\mu}{\norm{r_c}^3}}$ in $\text{rad}\cdot s^{-1}$, $\mu = 398600.4418 \ \text{km}^{3}s^{-2}$ is the Earth's standard gravitational parameter and $r_c$ is the radius of the chief's circular orbit.

\subsection{Attitude Dynamics - Chief Frame} \label{sec:new_rotation_dynamics}
Note the rotation $\rotmat{D}{O}$ applied to the deputy thrust vector $F^{\coordframe{D}}_d$ in \eqref{eq:CWdynamics_translational}. Both frames $\coordframe{O}$ and $\coordframe{D}$ are rotating with respect to the inertial frame $\coordframe{E}$. The angular velocity equations are
%\begin{align*}
$\angularvel{E}{D}{O} := (\omega_1 \ \omega_2 \ \omega_3)^{\top}$,  
$\angularvel{O}{D}{O} := (\delta\omega_1 \ \delta\omega_2 \ \delta\omega_3)^{\top}$,
and
$\angularvel{E}{O}{O} := (0 \ 0 \ n)^{\top}$. 
%\end{align*}
The deputy external torque vector in the $\coordframe{O}$ frame is $\tau^{\coordframe{O}} := (\tau_1 \ \tau_2 \ \tau_3)^{\top}$ and from assumption A6 the deputy inertia matrix in the deputy-fixed frame is $$\inertia{D} = \begin{pmatrix}
J_1 & 0 & 0 \\ 0 & J_2 & 0 \\ 0 & 0 & J_3
\end{pmatrix}.$$

The angular velocity of the $\coordframe{D}$ frame relative to the $\coordframe{O}$ frame is 
$\angularvel{O}{D}{E} = \angularvel{E}{D}{E} - \angularvel{E}{O}{E}$,
with the time derivatives given by 
\begin{equation}
\label{eq:rel_ang_vel_inertial}
\dotangularvel{O}{D}{E} = \dotangularvel{E}{D}{E} - \dotangularvel{E}{O}{E}.
\end{equation}
From \eqref{eq:rotation_velocity_a} and \eqref{eq:rotation_velocity_b} we yield the relations 
\begin{align*}
\dotangularvel{O}{D}{E} &= \rotmat{O}{E}\skewop{\angularvel{E}{O}{O}}\angularvel{O}{D}{O} + \rotmat{O}{E}\dotangularvel{O}{D}{O} \\
\dotangularvel{E}{O}{E} &= \rotmat{O}{E}\underbrace{\skewop{\angularvel{E}{O}{O}}\angularvel{E}{O}{O}}_{=0} + \rotmat{O}{E}\underbrace{\dotangularvel{E}{O}{O}}_{=0} = 0  \\
\dotangularvel{E}{D}{E} &= \rotmat{D}{E}\underbrace{\skewop{\angularvel{E}{D}{D}}\angularvel{E}{D}{D}}_{=0} + \rotmat{D}{E}\dotangularvel{E}{D}{D}.
\end{align*}
Substituting these into a manipulation of \eqref{eq:rel_ang_vel_inertial} gives
the relation 
%\begin{equation}
%\label{eq:relframe_quat}
$\dotangularvel{O}{D}{O} =  \rotmat{D}{O}\dotangularvel{E}{D}{D} - \skewop{\angularvel{E}{O}{O}}\angularvel{O}{D}{O}$.
%\end{equation}
%with accompanying relative quaternion kinematics
%\begin{align}
%\label{eq:relframe_eta}
%\dotquatscalar{D}{O} &= \frac{1}{2}[\quatvector{D}{O}]^{\top}\angularvel{O}{D}{O} \\
%\label{eq:relframe_rho}
%\dotquatvector{D}{O} &= -\frac{1}{2}[\quatscalar{D}{O}\identity{3} + \skewop{\quatvector{D}{O}}]\angularvel{O}{D}{O}. 
%\end{align}
Let the deputy body have inertia matrix $\inertia{D}$ as measured in the deputy-fixed frame with external control torque vector $\tau^{\coordframe{D}}$ being applied about the center of mass. From Euler's second law of motion we have
\begin{equation}
\label{eq:deputy_slew}    
\dotangularvel{E}{D}{D} = -\inertiainv{D}\skewop{\angularvel{E}{D}{D}}[\inertia{D}\angularvel{E}{D}{D}] + \inertiainv{D}\tau^{\coordframe{D}},
\end{equation}
where $\inertiainv{D} := [\inertia{D}]^{-1}$. Application of rotational transformation to \eqref{eq:deputy_slew} gives
$$\dotangularvel{O}{D}{O} =  \rotmat{D}{O}[-\inertiainv{D}\skewop{\angularvel{E}{D}{D}}[\inertia{D}\angularvel{E}{D}{D}] + \inertiainv{D}\tau^{\coordframe{D}}] - \skewop{\angularvel{E}{O}{O}}\angularvel{O}{D}{O},$$
which expands to
\begin{dmath}
\label{eq:ugly_ass_equation}
\dotangularvel{O}{D}{O} = \skewop{\angularvel{O}{D}{O}}\angularvel{E}{O}{O} + \inertiainv{O}(t)\tau^{\coordframe{O}} -  \inertiainv{O}(t)\big(\skewop{\angularvel{O}{D}{O}}[\inertia{D}\rotmat{O}{D}\angularvel{O}{D}{O}] + \skewop{\angularvel{O}{D}{O}}[\inertia{D}\rotmat{O}{D}\angularvel{E}{O}{O}] + \skewop{\angularvel{E}{O}{O}}[\inertia{D}\rotmat{O}{D}\angularvel{O}{D}{O}] + \skewop{\angularvel{E}{O}{O}}[\inertia{D}\rotmat{O}{D}\angularvel{E}{O}{O}]\big).
\end{dmath}
Here $\inertiainv{O} = \rotmat{D}{O}\inertiainv{D}\rotmat{O}{D}$ is a time-varying inertia matrix.

\subsection{Docking Configuration} \label{sec:docking_config}
To achieve a successful docking configuration, the deputy must reach a set of predefined relative translational and attitudinal states. Let $\quatdes{D}{O}$ be the quaternion representing the desired rotation from the deputy $\coordframe{D}$ frame to the CW $\coordframe{O}$ frame, and let $\quat{D}{O}$ be the actual (i.e., plant-state) rotation quaternion. Analogously, let $\angularveldes{O}{D}{O}$ be the desired relative angular velocity and $\angularvel{O}{D}{O}$ be the actual relative angular velocity. Lastly, let $\quaterr{D}{O} := \{\quatdes{D}{O}\}^{-1}\otimes\quat{D}{O}$ and $\angularvelerr{O}{D}{O} := \angularvel{O}{D}{O} - \angularveldes{O}{D}{O}$ respectively denote the error quaternion and error angular velocity. 

To achieve on-orbit attitudinal synchronization between both spacecraft, the aim is to drive $\quaterr{D}{O} \to q^{I}$ and $\angularvelerr{O}{D}{O} \to \mathbf{0}_3$. In the ARPOD problem, $\quatdes{D}{O} = q^{I}$ and $\angularveldes{O}{D}{O} = \mathbf{0}_3$, which results in the attitudinal error 
kinematics~$\dotquatscalarerr{D}{O} = \frac{1}{2}[\quatvectorerr{D}{O}]^{\top}\angularvelerr{O}{D}{O}$
and~$\dotquatvectorerr{D}{O} = -\frac{1}{2}[\quatscalarerr{D}{O}\identity{3} + \skewop{\quatvectorerr{D}{O}}]\angularvelerr{O}{D}{O}$. 
%
%\begin{align}
%\label{eq:error_eta}
%\dotquatscalarerr{D}{O} &= \frac{1}{2}[\quatvectorerr{D}{O}]^{\top}\angularvelerr{O}{D}{O} \\
%\label{eq:error_rho}
%\dotquatvectorerr{D}{O} &= -\frac{1}{2}[\quatscalarerr{D}{O}\identity{3} + \skewop{\quatvectorerr{D}{O}}]\angularvelerr{O}{D}{O}. 
%\end{align}
Relative translational states required for docking are $\delta r^{\coordframe{O}} = \textbf{0}_{3}$ and $\delta \dot{r}^{\coordframe{O}} = \textbf{0}_{3}$. The state vector of interest is
\begin{equation}
x \coloneqq \Big([\delta r^{\coordframe{O}}]^{\top}, \ [\delta\dot{r}^{\coordframe{O}}]^{\top}, \ \quatscalarerr{D}{O}, \ [\quatvectorerr{D}{O}]^{\top}, \ [\angularvelerr{O}{D}{O}]^{\top}\Big)^{\top} \in \chi
\end{equation}
and the objective docking state be
\begin{equation}
\label{eq:docking}
x_d \coloneqq  ([\mathbf{0}_3]^{\top}, \ [\mathbf{0}_3]^{\top}, \ 1, \ [\mathbf{0}_3]^{\top}, \ [\mathbf{0}_3]^{\top})^{\top} \in \chi.
\end{equation}
This vector~$x_d$ 
indicates that the frame~$\coordframe{O}$ has the same origin, linear velocity, orientation, and angular velocity as frame~$\coordframe{D}$. 
Let the control vector of interest in frame $\coordframe{O}$ be
%\begin{equation}
%\label{eq:inputs}
$u \coloneqq  ([F^{\coordframe{D}}_d]^{\top}, \ [\tau^{\coordframe{D}}]^{\top})^{\top} \in \mathcal{U}$
%\end{equation}
and the objective inputs be
%\begin{equation}
%\label{eq:inputsDesired}
$u_d \coloneqq  ([\mathbf{0}_3]^{\top}, \ [\mathbf{0}_3]^{\top})^{\top} \in \mathcal{U}$.
%\end{equation}
Let us define~$z(k) \coloneqq [u(k)^\top \ x(k)^\top]^\top$ and $z_d \coloneqq [u_d^\top \ x_d^\top]^\top$.
The next section uses this model to solve the ARPOD problem using
time-constrained MPC. 
